Regularization of Nonlinear Inverse Problems -- From Functional Analysis to Data-Driven Approaches

The focus of this book is on the analysis of regularization methods for solving \emph{nonlinear inverse problems}. Specifically, we place a strong emphasis on techniques that incorporate supervised or unsupervised data derived from prior experiments. This approach enables the integration of data-driven insights into the solution of inverse problems governed by physical models. \emph{Inverse problems}, in general, aim to uncover the \emph{inner mechanisms} of an observed system based on indirect or incomplete measurements. This field has far-reaching applications across various disciplines, such as medical or geophysical imaging, as well as, more broadly speaking, industrial processes where identifying hidden parameters is essential.

==> header.tex <==
\newif\ifdgruyter
\newif\ifsolutions
\newif\ifcomments


%% uncomment for dgruyter build
%%   comment for standard build
%\dgruytertrue


%% uncomment for showing solutions
\solutionstrue


%% uncomment for showing comments
%\commentstrue


%% show citation keys
%\usepackage{showkeys}


\ifx\directlua\undefined\ifx\XeTeXcharclass\undefined
  %\usepackage[utf8]{inputenc}                           %pdftex engine
  \else\RequirePackage[no-math]{fontspec}[2017/03/31]\fi %xetex engine
  \else\RequirePackage[no-math]{fontspec}[2017/03/31]\fi %luatex engine

\usepackage{fontenc}
\usepackage[utf8]{inputenc}
\usepackage{xcolor}
\usepackage{tcolorbox}
\tcbuselibrary{skins}

\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage{algpseudocode}
\usepackage{dsfont}

\usepackage{tikz}
\usetikzlibrary{math,calc,intersections,arrows.meta,tikzmark,positioning,decorations.pathreplacing,shadings}
\usepackage{pgfplots}
\usepackage{comment}

\usepackage{xr-hyper}

\ifdgruyter
  \usepackage[small]{dgruyter}
\else
  \usepackage{amsthm}
  \makeatletter
  \newcommand{\subtitle}[1]{\gdef\@subtitle{#1}}
  \newcommand{\@subtitle}{}
  \newcommand{\classification}[2][]{\gdef\@classification{#2}}
  \newcommand{\@classification}{}
  \renewcommand{\maketitle}{%
  \begin{titlepage}
      \centering
      {\LARGE \textbf{\@title} \par}
      \vspace{1em}
      {\large \textit{\@subtitle} \par}
      \vspace{2em}
      {\large \textbf{\@author} \par}
      \vfill
      {\noindent\textbf{Mathematics Subject Classification 2010:}\\\@classification \par}
      \vspace{2em}
  \end{titlepage}
  }
  \makeatother
  \newcommand{\dedication}[1]{#1}
  \usepackage[pdftex,colorlinks=true,linkcolor=blue,citecolor=green,urlcolor=blue,bookmarks=true,bookmarksnumbered=true]{hyperref}
  \hypersetup
  {
    bookmarksnumbered,
    breaklinks,
    pdfborderstyle=,
    colorlinks,
    citecolor=[rgb]{0,.65,0},
    linkcolor=[rgb]{0,0,.5},
    urlcolor=[rgb]{0,0,.5},
    pdfauthor={Otmar Scherzer},
  }
  %\newtheorem{proof}{Proof}
  \usepackage{amsmath,amssymb,dsfont}
\fi

\usepackage{suffix}
\WithSuffix\newcommand\boxed*[1]{\boxed{#1}}

\usepackage{subcaption}

\usepackage{imakeidx}

\usepackage{url}

\newcommand{\dom}[1]{{\cal D}(#1)}
\newcommand{\range}[1]{{\cal R}(#1)}
\newcommand{\inner}[2]{\left<#1,#2\right>}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norms}[1]{\|#1\|}
\newcommand{\abss}[1]{|#1|}

\newcommand{\X}{{\tt X}}
\newcommand{\Y}{{\tt Y}}

\newcommand{\y}{{\tt y}}
\newcommand{\m}{{\tt m}}
\newcommand{\n}{{\tt n}}

\newcommand{\yd}{\y^\delta}
\newcommand{\oby}{{\overline{\y}}}

\newcommand{\x}{{\tt x}}
\newcommand{\z}{{\tt z}}

\newcommand{\h}{{\tt h}}
\newcommand{\f}{{\tt f}}

\newcommand{\U}{{\tt U}}
\newcommand{\xk}{\x_{k}}
\newcommand{\xkp}{\x_{k+1}}
\newcommand{\xkpp}{\x_{k+1/2}}
\newcommand{\xkd}{\x_{k}^\delta}
\newcommand{\xkpd}{\x_{k+1}^\delta}
\newcommand{\xkppd}{\x_{k+1/2}^\delta}
\newcommand{\xad}{\x_{\alpha}^\delta}
\newcommand{\xademn}{\x^{\alpha,\delta,\eta}_{\ttm,\ttn}}
\newcommand{\xa}{\x_{\alpha}}
\newcommand{\xdag}{\x^\dagger}
\newcommand{\obx}{{\overline{\x}}}
\newcommand{\xknds}{\x_{k_n}^{\delta_n}}
\newcommand{\xknd}{\x_k^{\delta_n}}
\newcommand{\hk}{{\tt h}_k}

\newcommand{\lkd}{\lambda_{k}^\delta}
\newcommand{\mkd}{\mu_{k}^\delta}
\newcommand{\lkpd}{l_{k+1}^\delta}
\newcommand{\lkppd}{l_{k+1/2}^\delta}
\newcommand{\Ukd}{\U_{k}^\delta}

\newcommand{\T}{{\mathcal{T}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\id}{{\mathcal I}}

\newcommand{\ve}{\varepsilon}

\newcommand{\bx}{{\vec{x}}}
\newcommand{\by}{{\vec{y}}}
\newcommand{\bw}{{\bf w}}

\newcommand{\vx}{{\vec{x}}}
\newcommand{\vs}{{\vec{s}}}
\newcommand{\vH}{{\vec{H}}}
\newcommand{\vt}{{\vec{t}}}
\newcommand{\vr}{{\vec{r}}}

\newcommand{\vu}{{\bf u}}
\newcommand{\vv}{{\bf v}}
\newcommand{\vh}{{\vec{h}}}

% euler number
\newcommand{\e}{\mathrm e}

\newcommand{\vy}{{\vec{y}}}
\newcommand{\vp}{{\vec p}}
\newcommand{\vq}{{\vec q}}
\newcommand{\bP}{{\tt P}}
\newcommand{\vfm}{{\vec{\tt{h}}}}
\newcommand{\fun}{{{\tt x}}}

\newcommand{\su}{s}

\newcommand{\vw}{\vec{w}}
\newcommand{\vz}{\vec{z}}
\newcommand{\vzm}{{\bf{z}}}
\newcommand{\scinn}[1]{S_{#1}} %{S^C_{#1}}
\newcommand{\wcinn}[1]{\psi_{#1}}%{\psi^C_{#1}}
\newcommand{\interval}{\texttt{I}}
\newcommand{\quader}{\texttt{Q}}

%%% Random
\newcommand{\prob}{\mathbb{P}}
\newcommand{\probm}{\mathtt{P}}
\newcommand{\cprob}{{\mathbb{P}^c}\!\!\!}
\newcommand{\state}{{\textsf s}}
\newcommand{\stater}{{\textsf r}}
\newcommand{\staterv}{{\textsf S}}
\newcommand{\obse}{{\textsf o}}
\newcommand{\observ}{{\textsf O}}

\newcommand{\vl}{{\vec{\lambda}}}

% Specific activation functions
\newcommand{\sigmoid}{\sigma_g}
\newcommand{\tanhac}{\sigma_h} % tanh for hidden state/candidate
\newcommand{\tanhcell}{\sigma_c} % tanh for cell state output


\postdisplaypenalty=1000
\widowpenalty=1000
\clubpenalty=1000
\displaywidowpenalty=1000
%\setlength{\parskip}{.2ex}
\renewcommand{\labelenumi}{\textit{(\roman{enumi})}}
\renewcommand{\theenumi}{\textit{(\roman{enumi})}}

\newcommand{\N}{\mathds{N}}
\newcommand{\ZN}{\mathds{Z}}
\newcommand{\R}{\mathds{R}}
\newcommand{\C}{\mathds{C}}

\definecolor{colorhigh}{gray}{0.95}
\definecolor{colorhighborder}{gray}{0.60}
\newlength{\highborderwidth}\setlength{\highborderwidth}{0.5pt}
\newlength{\emphdistancealg}\setlength{\emphdistancealg}{2.1ex}
\newlength{\emphheightalg}\setlength{\emphheightalg}{3.1ex}
\tikzstyle{emphinlinelinestyle}=[draw=colorhighborder,line width=\highborderwidth]

\newcommand{\emphinlinealg}[2]{%
\tikzset{tikzmark suffix={emphinlinealg-#1}}%
\tikzmark{ebeg}#2\tikzmark{eend}%
}

\newcommand{\emphinlinealgdraw}[1]{%
\tikzset{tikzmark suffix={emphinlinealg-#1}}%
\tikz[overlay,remember picture]{
\coordinate (b) at ($ (pic cs:ebeg) + (-0.4ex,\emphdistancealg) $);
\coordinate (b2) at ($ (b) - (0ex,\emphheightalg) $);
\coordinate (e) at ($ (pic cs:eend) + (+0.4ex,\emphdistancealg) $);
\coordinate (e2) at ($ (e) - (0ex,\emphheightalg) $);
\draw[draw=none,fill=colorhigh] (b) -- (e) -- (e2) -- (b2) -- cycle;
\draw[emphinlinelinestyle] (b) -- (e);
\draw[emphinlinelinestyle] (b2) -- (e2);
}}

\usepackage{xparse}
\usepackage{environ}
\ExplSyntaxOn
\DeclareExpandableDocumentCommand{\floor}{m}
 {
  \fp_eval:n { floor ( #1 ) }
 }
\ExplSyntaxOff
\newcommand{\emphcenter}{%
\leftskip=0cm plus 0.5fil \rightskip=0cm plus -0.5fil%
\parfillskip=0cm plus 1fil \noindent}
\newlength{\inputlength}
\newcounter{breakerlines}
\newcommand{\emphboxwidth}[2]
{\begin{tcolorbox}[
  colback=colorhigh,
  center,
  valign=center,
  colframe=black,
  boxrule=0pt,
  enhanced,
  frame hidden,
  arc=0pt,
  left=2.0pt,
  right=2.0pt,
  top=2.0pt,
  bottom=2.0pt,
  borderline north={\highborderwidth}{0pt}{colorhighborder},
  borderline south={\highborderwidth}{0pt}{colorhighborder},
  width=#2,
% after skip=5pt,
]\emphcenter#1
\end{tcolorbox}}


\newcommand{\specialemphbox}[1]
{\begin{tcolorbox}[
  colback=colorhigh,
  center,
  valign=center,
  colframe=black,
  boxrule=0pt,
  enhanced,
  frame hidden,
  arc=0pt,
  left=2.0pt,
  right=2.0pt,
  top=2.0pt,
  bottom=2.0pt,
  borderline north={0.5pt}{0pt}{black},
  borderline south={1pt}{0pt}{black},
  width=\linewidth,
% after skip=5pt,
]\emphcenter#1
\end{tcolorbox}}

\ifcomments
	\newcommand{\commentO}[1]{\textcolor{red}{#1}}
	\newcommand{\commC}[1]{\textcolor{blue}{#1}}
	\newcommand{\commentC}[1]{\textcolor{blue}{\textbf{Clemens:} #1}}
	\newcommand{\commentS}[1]{\textcolor{orange}{\textbf{Christina:} #1}}
	\newcommand{\commentCS}[1]{\textcolor{violet}{\textbf{Cong:} #1}}
	\newcommand{\commentB}[1]{\textcolor{olive}{\textbf{Bochra:} #1}}
\else
	\newcommand{\commentO}[1]{}
	\newcommand{\commC}[1]{}
	\newcommand{\commentC}[1]{}
	\newcommand{\commentS}[1]{}
	\newcommand{\commentCS}[1]{}
	\newcommand{\commentB}[1]{}
\fi

%\newcommand{\commentO}[1]{\errmessage{no comments!}}
%\newcommand{\commentC}[1]{\errmessage{no comments!}}
%\newcommand{\commentS}[1]{\errmessage{no comments!}}

%' detect if having csc bibliography
%\makeatletter
%\begingroup
%\endlinechar=-1\everyeof{\noexpand}
%\edef\x{\endgroup\def\noexpand\bibinputs{\@@input|"kpsewhich infmath.bib" }}\x
%\makeatother
%\ifx\bibinputs\empty\else\def\havecscbib{}\fi

\usepackage[backend=biber,maxnames=10,backref=true,hyperref=true,giveninits=true,safeinputenc]{biblatex}
\addbibresource{csc.bib}
\addbibresource{local.bib}
\addbibresource{unpublished.bib}
%\ifdefined\havecscbib
%    \addbibresource{journals.bib}
%    \addbibresource{articles.bib}
%    \addbibresource{books.bib}
%    \addbibresource{data.bib}
%    \addbibresource{incollection.bib}
%    \addbibresource{inproceedings.bib}
%    \addbibresource{proceedings.bib}
%    \addbibresource{preprints.bib}
%    \addbibresource{theses.bib}
%    \addbibresource{infmath.bib}
%    \addbibresource{infmath_books.bib}
%    \addbibresource{infmath_report.bib}
%    \addbibresource{infmath_theses.bib}
%    \ifdefined\extract
%    \else
%        \addbibresource{local.bib}
%        \addbibresource{unpublished.bib}
%    \fi
%\else
%    \ifdefined\extract
%      \errmessage{cannot extract without detected csc bibliography}
%    \fi
%    \addbibresource{csc.bib}
%    \addbibresource{local.bib}
%    \addbibresource{unpublished.bib}
%\fi

\DeclareSourcemap{
  \maps[datatype=bibtex]{
    \map{
      \step[fieldsource = doi, final]
      \step[fieldset = url, null]
    }
    \map{
      \step[fieldset = note, null]
    }
  }
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Declare Math Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Real part
\let\RE\Re
\let\Re=\undefined
\DeclareMathOperator{\Re}{\RE e}
% Imaginary part
\let\IM\Im
\let\Im=\undefined
\DeclareMathOperator{\Im}{\IM m}
% Support
\DeclareMathOperator{\supp}{supp}
% Sign
\DeclareMathOperator{\sign}{sign}
% Absolute Value
\newcommand{\abs}[1]{\left|#1\right|}
%\newcommand{\abss}[1]{|#1|}
% Set
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\sets}[1]{\{#1\}}
% Nullspace
\newcommand{\nsp}[1]{\mathcal{N}(#1)}
% Operator
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\spann}{span}
\DeclareMathOperator{\Lip}{Lip}

\newcommand{\op}[1]{{F[#1]}}
\newcommand{\opdis}[2]{{F_{#1}[#2]}}
\newcommand{\opo}{F}

\newcommand{\opd}[1]{{F'[#1]}}

\newcommand{\lop}[1]{{P[#1]}}
\newcommand{\lopo}{P}

\newcommand{\nop}[1]{{N[#1]}}
\newcommand{\nopo}{N}

\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\no}{{\tt{N}}}

\newcommand{\be}{{\mathbf{e}}}
\newcommand{\bE}{{\mathbf{E}}}

\renewcommand{\i}{{\tt{i}}}
\renewcommand{\exp}{{\tt{e}}}

\newcommand{\sinc}{\text{sinc}}

\newcommand{\ttm}{{\tt m}}
\newcommand{\ttn}{{\tt n}}

\newcommand{\degree}{{\hat m}} %{\tt{m}}}

\newcommand{\noc}{{\tt{M}}}
\newcommand{\dimlimit}{{\noc_*}} %{\tt{m}}}

\newcommand{\deep}[1]{{D\left[#1\right]}}

\newcommand{\ALNN}{{\bf ALNN}\,}
\newcommand{\RQNN}{{\bf RQNN}\,}
\newcommand{\RePU}{{\bf RePU}\,}
\newcommand{\ReLU}{{\bf ReLU}\,}
\newcommand{\LReLU}{{\bf LeakyReLU}\,}
\newcommand{\ReLUs}{{\bf ReLU6}\,}
\newcommand{\RReLU}{{\bf RReLU}\,}
\newcommand{\PReLU}{{\bf PReLU}\,}
\newcommand{\HSh}{{\bf HardShrink}\,}
\newcommand{\HS}{{\bf HardSigmoid}\,}
\newcommand{\HT}{{\bf HardTanh}\,}
\newcommand{\HSw}{{\bf HardSwish}\,}
\newcommand{\LR}{{\bf LeakyReLU}\,}
\newcommand{\PR}{{\bf PReLU}\,}
\newcommand{\SoS}{{\bf SoftShrink}\,}
\newcommand{\SM}{{\bf Softmax}\,}
\newcommand{\Th}{{\bf Threshold}\,}
\newcommand{\LS}{{\bf LogSigmoid}\,}
\newcommand{\SP}{{\bf Softplus}\,}
\newcommand{\TS}{{\bf TanShrink}\,}
\newcommand{\CELU}{{\bf CELU}\,}
\newcommand{\ELU}{{\bf ELU}\,}
\newcommand{\SELU}{{\bf SELU}\,}
\newcommand{\Sig}{{\bf Sigmoid}\,}

\newcommand{\IRLI}{{\bf IRLI}\,}
\newcommand{\suIRLI}{{\bf s-IRLI}\,}
\newcommand{\sIRLI}{{\bf 2st-IRLI}\,}
\newcommand{\wUIRLI}{{\bf wu-IRLI}\,}
\newcommand{\cuIRLI}{{\bf cu-IRLI}\,}

\newcommand{\IRGN}{{\bf IRGN}\,}
\newcommand{\SIRGN}{{\bf s-IRGN}\,}
\newcommand{\wUIRGN}{{\bf wu-IRGN}\,}
\newcommand{\cuIRGN}{{\bf cu-IRGN}\,}
\newcommand{\ruIRGN}{{\bf ru-IRGN}\,}

\newcommand{\DeepONet}{Operator network\,}%{{\bf DeepONet}\,}
\newcommand{\deepONet}{operator network\,}

\newcommand{\Z}{{\mathtt Z}}

\newcommand{\vwm}{{\bf{w}}}
%\newcommand{\vfm}{{\bf{f}}}
\newcommand{\I}[1]{\mathcal{I}_{#1}}

%%% level set

\newcommand{\network}{{\tt s}} %\Psi
\newcommand{\mult}{\imath}
\newcommand{\multiphase}{{\mathrm{m}}}
\newcommand{\nnset}{{\tt S}} %\mathcal{N}
\newcommand{\levelfun}{{\tt l}} %\ell}}} %\phi
\newcommand{\nettwo}{{\tt t}} %\Psi
\newcommand{\nntwo}{{\tt T}} %\mathcal{D}
\newcommand{\affine}{{\tt a}} %\varphi


%%% Random

\newcommand{\randomv}{p}%{\mathbb P}}

\newcommand{\Alpha}{A}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% hyperref
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{aliascnt}

\newtheorem{lemma}{Lemma}[section]
\providecommand*{\lemmaautorefname}{Lemma}

\newaliascnt{remark}{lemma}
\newtheorem{remark}[remark]{Remark}
\aliascntresetthe{remark}
\providecommand*{\remarkautorefname}{Remark}

\newaliascnt{proposition}{lemma}
\newtheorem{proposition}[proposition]{Proposition}
\aliascntresetthe{proposition}
\providecommand*{\propositionautorefname}{Proposition}

\newaliascnt{corollary}{lemma}
\newtheorem{corollary}[corollary]{Corollary}
\aliascntresetthe{corollary}
\providecommand*{\corollaryautorefname}{Corollary}

\newaliascnt{theorem}{lemma}
\newtheorem{theorem}[theorem]{Theorem}
\aliascntresetthe{theorem}
\providecommand*{\theoremautorefname}{Theorem}

%\theorembodyfont{\normalfont}
\newaliascnt{definition}{lemma}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}
\providecommand*{\definitionautorefname}{Definition}

\newaliascnt{assumption}{lemma}
\newtheorem{assumption}[assumption]{Assumption}
\aliascntresetthe{assumption}
\providecommand*{\assumptionautorefname}{Assumption}

\newaliascnt{example}{lemma}
\newtheorem{example}[example]{Example}
\aliascntresetthe{example}
\providecommand*{\exampleautorefname}{Example}

\newaliascnt{notation}{lemma}
\newtheorem{notation}[notation]{Notation}
\aliascntresetthe{notation}
\providecommand*{\notationautorefname}{Notation}

\newaliascnt{convention}{lemma}
\newtheorem{convention}[convention]{Convention}
\aliascntresetthe{convention}
\providecommand*{\conventionautorefname}{Convention}

\newaliascnt{simple}{lemma}
\newtheorem{simple}[simple]{Simplification}
\aliascntresetthe{simple}
\providecommand*{\simpleautorefname}{Simplification}

\providecommand*{\algorithmautorefname}{Algorithm}

\newcounter{opq}
\setcounter{opq}{0}
\newtheorem{opq}[opq]{Open Question}
\providecommand*{\opqautorefname}{Open Question}
\renewcommand{\theopq}{\arabic{opq}}

\newcounter{exercise}
\setcounter{exercise}{0}
\newtheorem{exercise}[exercise]{Exercise}
\providecommand*{\exerciseautorefname}{Exercise}
\renewcommand{\theexercise}{\arabic{exercise}}

\ifsolutions
	\definecolor{univieBlue}{RGB}{0,99,166}
	\makeatletter
	\newenvironment{solution}
	{\par\noindent\color{univieBlue}\em{\bf\em Solution.}\par\nobreak\@afterheading}
	{\par\vspace{1em}}
	\makeatother
\else
 	\excludecomment{solution}
\fi

\def\chapterautorefname{Chapter}
\def\sectionautorefname{Section}
\def\subsectionautorefname{Section}


